Which Features are Learnt by Contrastive Learning? On the Role of Simplicity Bias in Class Collapse and Feature Suppression

Contrastive learning (CL) has emerged as a powerful technique for representation learning, with or without label supervision. However, supervised CL is prone to collapsing representations of subclasses within a class by not capturing all their features, and unsupervised CL may suppress harder class-relevant features by focusing on learning easy class-irrelevant features; both significantly compromise representation quality. Yet, there is no theoretical understanding of \textit{class collapse} or \textit{feature suppression} at \textit{test} time. We provide the first unified theoretically rigorous framework to determine \textit{which} features are learnt by CL. Our analysis indicate that, perhaps surprisingly, bias of (stochastic) gradient descent towards finding simpler solutions is a key factor in collapsing subclass representations and suppressing harder class-relevant features. Moreover, we present increasing embedding dimensionality and improving the quality of data augmentations as two theoretically motivated solutions to {feature suppression}. We also provide the first theoretical explanation for why employing supervised and unsupervised CL together yields higher-quality representations, even when using commonly-used stochastic gradient methods.

==> class_collapse_old.tex <==
\section{How Inductive bias Contributes to Class Collapse in Supcon}\label{sec: cc}
% \yx{replace test set class collapse with `poor representations on test set?' the issue was we can show exist minimizers that do not have test set cc. but we can't exactly show min norm has test set cc (we can only show it has bad representations)}


We say the model learns the subclass when its weight has a non-trivial alignment with $\vct{v}_2$, i.e., $\|\mtx{W}\vct{v}_2\|=\Omega(1)$ and produces highly separable embeddings on the population. Conversely, we say class collapse happens when the alignment when the alignment is small:
$$
\|\mtx{W}\vct{v}_2\|=O(\frac{\sigma_\xi}{\sqrt{mn}}) = o(1).
$$
\yx{try convergence rate of training linear head using GD and sample complexity of hard margin SVM}
\yx{or argue that this means class \emph{asymptotically} collapses}
\yx{definition}

The above implies that (1) the subclasses are not well separated in the embedding space since the distance between two examples with different subclass labels can be as small as $\|2\mtx{W}\vct{v}_2\|=o(1)$. 
% As a result a very small perturbation at $\vct{v}_2$ no linear classifier can perform beyond random guess in the embedding space; 
(2) the distinguishability of subclasses is arguably at odds with generalization since the latter usually improves as sample size increases or noise decreases. 

\yx{actually we are able to add downstream performance to each of the theorem showing subclass separability except for theorem \ref{thm: minimizer_with_cc}. We can also define class/subclass separability and argue that when the there is a small perturbation on embeddings at test time subclasses are not separable in \ref{thm: minimizer_with_cc}}

We make two key observations through theory and numerical experiments
\begin{itemize}
    \item[1.] [Theory] Not all global minimizers exhibit class collapse. But the \emph{minimum norm} minimizer does.
    \item[2.] [Theory] When the model is trained using gradient descent (GD), some subclasses are \emph{provably} learned early in training. [Numerical experiments] However, those subclasses will eventually be unlearned. In other words, gradient descent converges to minimizers that exhibit class collapse.\looseness=-1
\end{itemize}
These observations together suggest that class collapse, which has been observed in practice where certain gradient based algorithms are used to minimize the loss, can not be explained by simply analyzing the loss function. This highlights the importance of studying the dynamics and inductive bias of training algorithms in contrastive learning. We will discuss these in more details. \looseness=-1


\begin{figure*}[!t]
\centering
\subfigure[epoch 0]{
\includegraphics[width=0.21\textwidth]{figures/class_collapse/p3/embedding_epoch[-1].eps}
	}
\subfigure[epoch 45]{
\includegraphics[width=0.21\textwidth]{figures/class_collapse/p3/embedding_epoch[45].eps}
	}
 \subfigure[epoch 60]{
\includegraphics[width=0.21\textwidth]{figures/class_collapse/p3/embedding_epoch[60].eps}
	}
 \subfigure[epoch 100]{
\includegraphics[width=0.21\textwidth]{figures/class_collapse/p3/embedding_epoch[100].eps}
	}
    \caption{Visualization of the embedding space at different epochs. We let $p=3$ so that we can see the whole embedding space from a 3D plot. Other parameters: $n=1000, m=5, d=2000, K=4, \phi_1=\phi_2=\phi_3=\phi_4=1, \mu=1, \sigma=2, \sigma_0=0.001, \eta=0.05$. Colors represent combinations of class and subclass labels $(y, y_\sub)$. We use test examples for the plots. At epoch 45, the four groups of examples are well separated in the embedding space. However groups in the same classes are merged afterwards. }
    \label{fig: cc_embedding}
\end{figure*}

\begin{figure}[!t]
    \centering
 \subfigure[$p=3$]{
\includegraphics[width=0.21\textwidth]{figures/class_collapse/p3/proj_v.eps}
}
 \subfigure[$p=500$]{
\includegraphics[width=0.21\textwidth]{figures/class_collapse/p500/proj_v.eps}
}
\vspace{-.3cm}
    \caption{$\|\mtx{W}_t \vct{v}_1 \|$ and $\|\mtx{W}_t \vct{v}_2 \|$ at different epochs. Both features are learned early in training, but $\vct{v}_2$ is unlearned later.}
    \label{fig: cc_alignment}
\end{figure}



%\subsection{Minimizing the $\mathcal{L}_\supcon$ does not necessarily lead to class collapse unless with certain inductive bias}\label{sec: cc_not_necessarily}

\subsection{Minimizing the $\mathcal{L}_\supcon \not \Rightarrow $ Class Collapse}
%\PYB{The subsection title has double negatives - hard to parse }

Firstly we prove that in the high-dimensional case there exist global minimizers that learns the subclasse feature $\vct{v}_2$ and outputs embeddings with infinitesimal overlap between subclasses on the population.\looseness=-1
\begin{theorem}\label{thm: minimizer_without_cc}
With probability at least $1-O(\frac{m^2n^2}{d})=1-o(1)$, there exist $\mtx{\Theta}^*=[\mtx{W}^*~~ \vct{b}^*]$ such that $\mtx{\Theta}^*\in \min_{\mtx{\Theta}}\mathcal{L}_\supcon(\mtx{\Theta})$ and $\|\vct{W}^*\vct{v}_2\|=\Omega(1)$ . \yx{either drop the below or add separability to every theorem} Moreover
\begin{align}
    \nonumber
    \exists \vct{\beta}, ~s.t.~  \Pr_{(\vct{x},y, y_\sub)\sim\mathcal{D}_\orig}(y_\sub\vct{\beta}^\top \mtx{W}\vct{x}>0 |y ) = 1-o(1).
\end{align}
\end{theorem}
\todoblue{prove the separability part}
We prove the theorem in Appendix \ref{apdx: prop_minimizers}. Lemma \ref{lemma: SVD_perturb} implies that, due to the high-dimensionality, the noise vectors have non-trivial effects on the empirical covariance matrix by rotating its kernel space such that the kernel space has a $\Theta(\frac{\sigma_\xi}{\sqrt{mn}})$ alignment with the subclass feature. And since the minimizers can behave arbitrarily on this kernel space, without any additional restriction, they can have any alignment with the subclass feature.

\subsection{Minimizing the $\mathcal{L}_\supcon$ $+$ Inductive Bias Towards Simplicity\yx{Minimum Norm?} $\implies$ Class Collapse}

However, below we show that, the minimum norm minimizer does exhibit class collapse, in the sense that its alignment with the subclass feature is small (Theorem \ref{thm: minimizer_with_cc}) \yx{replace test set class collapse with `poor representations?'}
\begin{theorem}\label{thm: minimizer_with_cc}
Let $\mtx{\Theta}^{**}=[\mtx{W}^{**}~~ \vct{b}^{**}]$ be the minimum norm minimizer of $\mathcal{L}_\supcon$, i.e.,
$$
\mtx{\Theta}^{**} = \arg\min_{\mtx{\Theta^*}} \| \mtx{\Theta}^* \|_F ~s.t.~ \mtx{\Theta}^*\in\arg\min_{\mtx{\Theta}} \mathcal{L}_\supcon(\mtx{\Theta}).
$$
Then with probability at least $1-O(\frac{m^2n^2}{d})=1-o(1)$, $\|\mtx{W}^{**} \vct{v}_1 \|=\Theta(1)$ but $\|\mtx{W}^{**} \vct{v}_2 \|=O(\frac{\sigma_\xi}{\sqrt{mn}}) = o(1)$. 
% Moreover, $\forall \vct{\beta}\in\mathbbm{R}^p$
% \begin{align}
%     \nonumber
%     \Pr_{ \substack{(\vct{x},y, y_\sub)\sim\mathcal{D}_\orig, \\
%     \epsilon\sim\mathcal{N}(0,\sigma_\epsilon^2) } }(y_\sub\vct{\beta}^\top \mtx{W}(\vct{x}+ \epsilon \vct{v}_2)>0 |y ) \leq 1+o(1),
% \end{align}
% as long as $\sigma_\epsilon^2$ 
\end{theorem}


\subsection{Intriguing properties of GD}
We now investigate the case where $\mathcal{L}_\supcon$ is minimized by GD. We see this as a step toward understanding class collapse in practice where certain optimization algorithms are used to minimize the loss. As we will show below, our results raise an important question that can not be answered by any algorithm agnostic analysis of class collapse. 

We consider GD with a constant learning rate $\eta$. The weights are initialized from a Gaussian distribution, i.e., the initial weight $\mtx{\Theta}_0$ has each of its element drawn from $\mathcal{N}(0, \frac{\sigma_0^2}{d})$. And the weight at training epoch $t$ is given by
\begin{align}
    \nonumber
    \mtx{\Theta}_t = \mtx{\Theta}_{t-1} -\eta \nabla_{\mtx{\Theta}}\mathcal{L}_\supcon (\mtx{\Theta}_{t-1}).
\end{align}

% Two specific questions we explore here are: (1) Does class collapse happen in GD? (2) If it does, then how  
\paragraph{Early in training some subclasses are provably learned}
By analyzing the training dynamics of GD, we found that subclasses are learned sometime during training.  
\begin{theorem}\label{thm: early_in_training} Assume $\sigma_0\sqrt{\frac{p}{d}}=o(1)$ and $\sigma_\xi=o(1)$. If the subclass feature has a constant non-zero mean such that $1+\mu^2 > \phi_1^2 $, then with probability at least $1-O(\frac{m^2n^2}{d}+\frac{1}{\poly(p)})=1-o(1)$
the following holds
\begin{itemize}
    \item $\|\vct{W}_0\vct{v}_2\|=o(1)$.
    \item $\exists t=O(\ln(\frac{1}{\sigma_0} \sqrt{\frac{d}{p}}))$, s.t. $\| \mtx{W}_t\vct{v}_2\|=\Omega(1)$ 
\end{itemize}
\end{theorem}
The above theorem shows that there exists an epoch where the weight has non-trivial alignment with the subclass feature. We prove the result in Appendix \ref{apdx: early}. The key step of our analysis is showing that in the early phase of training GD aligns the weights with the first eigenvector of the covariance matrix of class centers. And this alignment grows exponentially faster than alignments with any other directions. When $1+\mu^2 >\phi_1^2$, the subclass feature has a constant projection onto the first eigenvector and is therefore learned by the model.  In the high level, \emph{not only does learning class features have no conflict with learning subclass features, it can even help the latter, although the latter is not enforced by the loss function. }  

Now the remaining question is, \emph{is the subclass information learned early in training maintained afterwards?} Analyzing the training dynamics in the later phase is essentially hard since there is a non-negligible third-order term in the gradient. However, we demonstrate experiments showing that the answer to the above question is \emph{No}.


\paragraph{Numerical evidence that class collapse eventually happens in GD} 
Interestingly, our experiments show that gradient descent converges to a minimizer that exhibits class collapse after learning the subclasses. We visualize the embeddings of test data at different epochs in Figure \ref{fig: cc_embedding} and plot the alignment between weights and class/subclass features in Figure \ref{fig: cc_alignment}. Subclasses are perfectly separated and the weights align with both $\vct{v}_1$ and $\vct{v}_2$ after around 100 epochs of training. Then the model starts unlearning $\vct{v}_2$ which causes the alignment to drop and subclasses are merged in the embedding space.

%This suggests that considering the inductive bias of the training algorithm is necessary for understanding class collapse in real settings.

\paragraph{Summary}
The above experimental results combined with our theoretical analyses raise an intriguing question:
\begin{center}
\emph{Given that class collapse is not necessary for minimizing the loss (by Theorem \ref{thm: minimizer_without_cc}), and the subclass feature has already been learned early in training (by Theorem \ref{thm: early_in_training}), which property (inductive bias) of GD makes it essentially unlearn the subclass feature? }
\end{center}
 We note that the answer can not be found in any of the existing analyses (e.g., \cite{cc_dissecting_scl_2021,cc_chen2022perfectlybalanced}) that are agnostic to the training algorithm. Theorem \ref{thm: minimizer_with_cc} suggests the possibility that such phenomenon can be explained by norm based inductive bias.  However, it still remains an open question which is the real inductive bias of GD. Note that the objective function here is different than supervised objectives (where the inductive bias of GD is understood better \todoblue{cite papers}), but can rather be reformulated as a matrix factorization objective (\todoblue{see Appendix}), where the debate on inductive bias (mostly about whether it is explained by norm or rank \todoblue{cite papers}, see more related works in Section \todoblue{related work}) is still ongoing. \looseness=-1


% This means that GD must have some sort of inductive bias toward such minimizers.
% In Appendix \ref{} we show that the Supcon loss can be written as a matrix factorization objective. (\todoblue{say that the inductive bias of GD on matrix factorization is still an open problem ...}) \todoblue{say that given our previous theory, this can not be explained by existing works that only look at population loss.}
% \looseness=-1 \

% \todoblue{for the numerical experiments, we can also report the performance of the constructed minimizer that learns subclasses}

% This, combined with our empirical observation in Figure \ref{}, means that there is a phase transition from learning subclasses to unlearning subclasses in training. We have characterized the first phase while the second phase is only empirically observed. Studying the second phase is important future work which could help understand how the inductive bias of training algorithm leads to class collapse. 

All the phenomena presented in this section are observed in real settings as we will see in Section \ref{sec: experiments} \todoblue{}. Thus addressing the above question is a key to understanding and improving supervised contrastive learning in practice.

\subsection{Extensions of theorems} 
It worth noting that our theoretical results are not an artifact of the specific data distribution we considered but are instead very generalizable. As we show in \todoblue{Appendix}, all the Theorems hold when the noise is Gaussian, and Theorem \ref{thm: minimizer_with_cc} can be extended to multi-class setting with a different proof technique \todoblue{@Eric, is this true?}. We defer the extensions to the Appendix. 


\section{Feature suppression in Unsupcon}
\todoblue{briefly explain what is feature suppression}

\yx{definition of feature suppression}

 In practice there are many different possible sources of feature suppression. Here we present two variants of feature suppression and explore the interplay between dimensionality of the output space, strength and dimensionality of class-irrelevant features and data augmentation. Moreover, neither variant can be explained without incorporating inductive bias. \looseness=-1
 
 % In the first variant, the easy-to-learn (indicated by magnitude of features) and class-irrelevant features suppress the class feature when the output space is limited. 


\subsection{Feature suppression due to easy irrelevant features and limited embedding space}
In Theorem \ref{thm: FS_1}, we show that the easy-to-learn (with easiness indicated by how much the features separate examples or the strength of the features) and class-irrelevant features can suppress the class feature when the output space is limited. \looseness=-1

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/feature_suppresion/fs_experiment.pdf}
    \label{fig: fs_embedding_space}
    \caption{Effect on Embedding Size Feature Suppression (MNIST RandBit Dataset \cite{chen2021intriguing})}
\end{figure}

% \yx{In the theorem .}

% \sj{Address that under both augmentations the augmentation distance between points in the same cluster is similar with not too large noise}

\begin{theorem}\label{thm: FS_1}[Feature Suppresion 1]
Assume $p\leq K$. Let $L$ be the $(K+1)$-element tuple $\big[\frac{(1+\mu^2+\phi_2^2)+\sqrt{(1+\mu^2+\phi_2)^2-4\phi_2^2} }{2}, \phi_1^2,$\\
$ 
\frac{(1+\mu^2+\phi_2^2)-\sqrt{(1+\mu^2+\phi_2)^2-4\phi_2^2} }{2}$,
$ \frac{\phi_3^2}{\sqrt{K-2}}, \dots, \frac{\phi_K^2}{\sqrt{K-2}} \big]$. If $\phi_1$ is not among the $p$ largest in $L$, then with probability at least $1-O(\frac{m^2n^2}{d})=1-o(1)$: (1) there exists a global minimizer $\mtx{\Theta}^*$ of $\mathcal{L}_\unsup$ such that $\| \vct{W}^* \vct{v}_1\| = \Omega(1)$, (2) However, the minimum norm minimizer $\mtx{\Theta}^{**}$ satisfies $\| \vct{W}^{**} \vct{v}_1\| = 0$.
\end{theorem}
\begin{remark}
We prove the theorem in Appendix \ref{apdx: FS}. Following the same analysis we can also show that when $\phi_1$ is among the $p$ largest, $\vct{v}_1$ is learned by the minimum norm minimizer and when $\phi_1$ is exactly on par with some other element as the $p$-th largest, there exist both minimum norm minimizers that learn and do not learn $\vct{v}_1$.
\end{remark}

% \todoblue{actually learning the class feature is also not guaranteed when the useless features are small. }

% \todoblue{it is hard to numerically compute the min norm minimizer in general when augmentation is not identity. since it is possible that the first $x$ ($x>p$) eigenvalues are equally large. and to naively find the minimum norm minimizer one has to examine all ${x \choose p}$ combinations. }

% \todoblue{show that numerically there are a lot of minimizers}

\yx{mention solutions}

To make it more straightforward, we consider the case where $\mu=0$. Then the elements except the first one in $L$ can be interpreted as the variance of examples at each coordinate $\vct{v}_k, k=1,2,\dots, K$, which indicates how separated examples are at each feature. They are also connected to the magnitudes of the features. Both notions suggest the `easiness' of the features. The theorem shows that when the embedding space is not large enough to represent all the $K$ features (which requires $K+1$ dimensions), the minimum norm minimizer only picks those with largest variance/magnitude. In practice, the embedding space in Unsupcon is relatively low-dimensional and thus the model can not fit all details about the inputs into the embedding space (even if input noises are not learned and the model itself has large capacity). As is suggested by our theorem, if the training algorithm prefers functions with certain simple structure, only the easiest features that can be mapped into the embedding space by less complex functions (e.g., smaller norm) are learned. The class features are suppressed if they happen to be not among the easiest ones.

\begin{figure}[!t]
    \centering
 \subfigure[$K=3, p=3$]{
\includegraphics[width=0.4\columnwidth]{figures/feature_suppresion/proj_v_3.eps}
}
 \subfigure[$K=50, p=50$]{
\includegraphics[width=0.4\columnwidth]{figures/feature_suppresion/proj_v_50.eps}
}
\vspace{-.1cm}
    \caption{{\bf The irrelevant feature suppresses the class feature when its variance is beyond the variance of the class feature (the red vertical line).} We let $d=2000, p=K$, $\phi_1=0.8, \phi_2=1, \mu=0$, $\frac{\phi_k^2}{K-2}>\phi_1, \forall k\in [K-1]$ and vary $\phi_K$. Thus whether $\phi_1^2$ is among the $p$ largest variances only depends on $\phi_K$. We train the linear model to convergence. Plots show that the alignment between the trained weights and $\vct{v}_1$ drops when $\phi_K$ increases. We report the average of 10 runs. The result diverges at $\frac{\phi_K^2}{K-2}= \phi_1^2$ indicating that the model can learn either $\vct{v}_1$ or $\vct{v}_K$ in this case.  \looseness=-1 }
    \label{fig: fs_alignment}
    \vspace{-.2cm}
\end{figure}

\paragraph{Numerical experiments with  GD.} 
Our theory for the minimum norm minimizer also matches the experimental results for models trained with GD. We let $p=K$ and set the values of $\phi$'s such that $\phi_1^2$ is among the smallest two variances. Then we vary $\phi_K$ and see how the trained weights align with $\vct{v}_1$. Consistent with Theorem 1, Figure \ref{fig: fs_alignment} shows that $\vct{v}_1$ is suppressed when $\frac{\phi_K^2}{K-2}> \phi_1^2$. Interestingly, we also see that the result at $\frac{\phi_K^2}{K-2}=\phi_1^2$ diverges, indicating that GD can find both minimizers that learn and do not learn $\vct{v}_1$ when the variances at $\vct{v}_1$ and $\vct{v}_K$ are the same.


% \subsection{Feature suppresion due to high-dimensional easy irrelevant features}

% proved assuming identity augmentation but confirmed with more realistic augmentation in experiments

\subsection{Feature suppression due to high-dimensional irrelevant features and imperfect augmentation}\label{sec: fs_2}
We show another version of feature suppresion which does not reply on the limited embedding space assumption but rather requires the irrelevant features to be (1) high dimensional and (2) less altered by data augmentation compared to the class feature. \looseness=-1

We consider the following data augmentation:
\begin{definition}[Data augmentation $\badaug{\cdot}$]
For a given example $\vct{x}=y \phi_1\vct{v}_1 + (y_\sub \phi_2+ \mu)\vct{v}_2 + \rho\phi_{k} \vct{v}_{k}+\vct{\xi}$ from $\hat{\mathcal{D}}_\orig$, \looseness=-1
\begin{align}
    \nonumber
    \badaug{\vct{x}} =& (y \phi_1 +\zeta')\vct{v}_1 + (y_\sub \phi_2+ \mu +\zeta'')\vct{v}_2\\
    \nonumber
    +& (\rho\phi_{k})\vct{v}_{k}+\vct{\xi}',
\end{align}
where $\zeta'\sim\mathcal{N}(0, \sigma_\zeta'^2)$, $\zeta''\sim\mathcal{N}(0, \sigma_\zeta''^2)$, $\sigma_\zeta'^2,\sigma_\zeta''^2 \neq 0$ and $\vct{\xi}'$ is a new random variable such that, given a fixed original noise vector $\vct{\xi}_i, \vct{\xi'} \sim \mathcal{N}(\vct{\xi}_i, \mtx{\Sigma}_{\vct{\xi}_i})$ with $\rank{\mtx{\Sigma}_{\vct{\xi}_i}} \leq  \frac{m}{2}$
\end{definition}

\eg{Explain generalizations: e.g., the $\vct{v_k}$ don't need to be orthogonal, only linearly independent, small noise along preserved directions}

Augmentation introduces slight noise to the class feature, but preserves irrelevant feature. Low rank augmentation of the noise guarantees that augmented noise are similar.

% \todoblue{@Eric Could you take a look and see if this definition works for your example of feature suppression? We already assume $K$ large enough, thus the n original examples already have distinct irrelevant features. Then we want to show with certain assumption on $\sigma_\zeta$'s, the class feature is suppressed. }

\begin{theorem}[Feature Suppression 2]\label{thm: FS_2}
If $K = \omega(n^2)$ and $d=\omega(m^2 n^2)$. Using augmentation $\badaug{\cdot}$, with probability $\geq 1-o(\frac{n^2m^2}{d} + \frac{1}{n}) = 1-o(1)$, the minimum norm minimizer $\mtx{\Theta}^*=[\mtx{W}^*, \vct{b}^*]$ satisfies $\|\mtx{W}^* \vct{v}_1\| = 0$.
\end{theorem}
\todoblue{this theorem explains another type of feature suppression that can not be attributed to the embedding dimensions. For example \cite{addressing_feature_suppression_2020} shows that increasing dimension does not improve performance on Colorful-Moving-MNIST.}
rephrase
\todoblue{example in practice: $\zeta$'s mimics the variation added to the useful features by augmentation. And some irrelevant features can be invariant to augmentations, (e.g., color is invariant to augmentations without color distortion) and discriminative enough to separate all the examples. Then, because of the bias toward simple solutions, the model not longer learns the relevant features even when there is remaining embedding space. }


% In this section we show that if there are a lot of easy-to-learn but class-irrelevant features and the output space is limited, the class feature can be suppressed in unsupervised contrastive learning. However, understanding this phenomenon also requires incorporating inductive bias of training algorithms. In high dimensional settings, feature suppression does not necessarily happen if no additional inductive bias is considered. Meanwhile numerical experiments show that feature suppresion is always observed when the model is trained by gradient descent.

% We also present a version of feature suppresion where random input noise suppresses the class features even if the output space can be arbitrarily large. And in this setting, we identify minimum rank and minimum norm as two inductive biases that could explain this phenomenon.
% \todo{it is interesting to see if early in training, class features can be learned.}

% \subsection{FS due to limited embedding space}
% \begin{theorem}
% Define $ \Phi =  \{ k: k\in[K], k\neq 1, \phi_k >\phi_1  \}$. If $p<K$ and $|\Phi| \geq p$, with probability at least \todoblue{}, the following holds
% \begin{itemize}
%     \item $\exists \mtx{\Theta}^*\in \argmin_{\mtx{\Theta}}\mathcal{L}_\unsup (\mtx{\Theta}) $ s.t. $\|\mtx{W}^*\vct{v}_1 \|= \Omega(1)$ and 
%     \begin{align}
%         \nonumber
%         \exists \vct{\beta}\in\mathbbm{R}^p,  ~s.t.~ \Pr_{(\vct{x},y, y_\sub) \sim \mathcal{D}_\orig }( \sign(f_{\mtx{\Theta}^*}(\vct{x})^{\top}\vct{\beta})= y) \geq 1 - o(1).
%     \end{align}
%     \item Let $\mtx{\Theta}^{**} $ be the minimum norm minimizer of $\mathcal{L}_\unsup (\mtx{\Theta}) $, we have $\|\mtx{W}^{**}\vct{v}_1 \|= \todoblue{}$ \todoblue{note that this should not be $f(\vct{v}_1)$} and 
%     \todoblue{analyze downstream task if we have time}
% \end{itemize}
% \end{theorem}

% \subsection{FS due to non-perfect augmentation}


\section{Combining Supcon and Unsupcon can avoid both class collapse and feature suppression}

\yx{Hanger: feature suppression is not even a problem if we assume access to labels. Maybe we should drop `avoid feature suppression'}

We now consider the following loss which is a weighted sum of the Supcon and Unsupcon loss functions \looseness=-1
\begin{align}
    \nonumber
    \mathcal{L}_{\intrpl, \beta} (\mtx{\Theta})= \beta \mathcal{L}_\supcon(\mtx{\Theta}) + (1-\beta)\mathcal{L}_\unsup(\mtx{\Theta}).
\end{align}
Loss functions at similar forms have been proposed recently for different purposes. For example, \cite{cc_chen2022perfectlybalanced} proposed a weighted sum of Supcon loss and class-conditional InfoNCE (which has similar effect as $\mathcal{L}_\unsup$ in our setting) to avoid class collapse. \cite{islam2021broad} empirically observed that the joint objective of cross-entropy/Supcon loss and Unsupcon loss leads to better transferability of the learned models over their supervised counterparts. However, we still lack a theoretical understanding of why this weighted sum can outperform (1) Supcon alone and (2) Unsupcon alone. Although \cite{cc_chen2022perfectlybalanced}'s analysis may shed lights on (1), they didn't analyze the minimizer of the loss (but instead bypassed it by evaluating constructed embeddings) and the anlaysis is agnostic to input, model and inductive bias, which, as we argued in Section \ref{sec: cc}, can't explain what has been observed in practice.  

With our in-depth analyses of class collapse and feature suppresion in previous sections, the benefit of the joint objective $\mathcal{L}_\intrpl$ has now come to light: the unsupervised term in $\mathcal{L}_\intrpl$ increases the chance of learning features that do not appear relevant to the labels but might be useful for downstream tasks, while the supervised term in $\mathcal{L}_\intrpl$ prioritizes the class feature in case it does not appear as easy-to-learn as other features.  Thus $\mathcal{L}_\intrpl$ can learn a rich representation that also preserves the class structure. We show below that with an appropriate choice of $\beta$, $\mathcal{L}_\intrpl$ can succeed where $\mathcal{L}_\supcon$ fails due to collapse and $\mathcal{L}_\unsup$ fails due to feature suppression 1. For simplicity we let $\mu=0$.
\looseness=-1
\begin{theorem}\label{thm: joint}
W.L.O.G., assume $\phi_3 \geq \phi_4 \geq \dots \geq \phi_K $. If $p\leq K$, $\phi_2^2 > \frac{\phi_{p-2}^2}{K-2} $ and $\phi_1^2 < \frac{\phi_{p-1}^2}{K-2}$, then by Theorem \ref{thm: minimizer_with_cc} the minimum norm minimizer of $\mathcal{L}_\supcon$ suffers from class collapse and by Theorem \ref{thm: FS_1} the minimum norm minimizer of $\mathcal{L}_\unsup$ suffers from feature suppresion. However, for constant $\beta \in (0, 1)$, the minimum norm minimizer of $\mathcal{L}_{\intrpl,\beta}$, denoted by $\mtx{\Theta}^*=[\mtx{W}^*~~ \vct{b}^*]$, satisfies $\|\mtx{W}^* \vct{v}_1 \|=\Omega(1)$ and $\|\mtx{W}^* \vct{v}_2 \|=\Omega(1)$. 
\end{theorem}

% The Unsupcon term increases the chance of learning the subclass feature. 


% Check this paper \cite{islam2021broad}, empirically stutied supcon+unsupcon loss. 'We further observe that the joint objective of self-supervised contrastive loss with cross-entropy/supervised-contrastive loss leads to better transferability of these models over their
% supervised counterparts. '

% Using unsupcon as a regularizer can improve the richness of the learned features. 

\section{Experiments}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/class_collapse/cc_well_learnt_subclasses.png}
    \label{fig: cc_well_learnt_subclasses}

    \caption{Subclasses Learnt Well and Unlearnt}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/class_collapse/cc_never_learnt_subclass.png}
    \label{fig: cc_well_learnt_subclasses}
    \caption{Subclass Never Learnt Well}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/class_collapse/cc_avg_subclass_acc.png}
    \label{fig: cc_well_learnt_subclasses}
    \caption{Average Subclass Accuracy}
\end{figure}

\section{Discussion and Conclusions}
Discuss how to generalize our result to the following setting if we have time (maybe not necessary)
\begin{align}
    \nonumber
    \vct{x} = y\phi_1\vct{v}_1+y_\sub \phi_2 \vct{v}_2 + \rho \phi_k\vct{v}_k + \vct{\zeta} + \vct{\xi},
\end{align}
where $\vct{\zeta}$ is a Gaussian vector in the span of features and $\vct{\xi}$ is Gaussian vector in the complement of the span of features.

Summarize the contributions again. 

==> intro-old.tex <==
\section{Introduction}

% \yx{a thought: can we say we study how inductive bias contributes to the failure modes of supcon and unsupcon?}

% Representation learning aims to
% %The goal of representation learning is to learn representations that succinctly capture all 
% capture the semantically relevant information from training examples \cite{cl_simclr}. 
Learning high-quality representations that generalize well to a variety of downstream prediction tasks has been a long-standing goal of machine learning \cite{hinton2006fast,ranzato2006efficient}.
Contrastive learning (CL) 
has emerged as an effective approach for solving this problem both with and without supervision \cite{cl_simclr, cl_chuang_debiased_2020, cl_grill_bootstrap_2020, khosla2020supervised}. 
Unsupervised CL learns representations of training examples by maximizing agreement between augmented views of the same example. Similarly, supervised CL maximizes agreement between augmented views of examples in the same class.
Despite their empirical success, %of these methods for many common tasks, 
both supervised and unsupervised contrastive learning 
% it has been observed that the representations learnt can often
fail to capture all the semantically relevant features in the data.
% despite sufficient model capacity. \yx{make it clear that we are discussing two separate problems} 
In particular, \textit{supervised} CL can fall prey to \textit{class collapse} % \yx{make it clear that it doesn't mean classes are not distinguishable}
\cite{cc_dissecting_scl_2021, cc_chen2022perfectlybalanced}, where representations of \textit{subclasses} within a class may no longer be distinguishable from each other, and yields a poor classification performance at the subclasses level.
%, \textit{collapsing} away any semantically relevant subclass information. This may render these representations useless in many practical use cases: for example, coarse to fine transfer learning. \cite{cc_issues} 
Similarly, \textit{unsupervised} CL can be afflicted with \textit{feature suppression} \cite{chen2021intriguing,shortcut2021_robinson}, where easy but class-irrelevant features suppress the learning of harder semantically relevant
% meaningful \yx{maybe we can use `relevant', since the suppressing features can also be semantically meaningful but just not relevant to the task} 
ones, and deteriorates generalizability of the obtained representations in general. \looseness=-1
% Therefore, class collapse and feature suppression must be addressed for contrastive learning to be a robust representation learning solution. 
% In both cases, the learned representations will not generalize well to a variety of downstream tasks.

% \PYB{I think we may need to make examples of what could go wrong when class collapse/feature suppression happens - e.g., failure to learn class-distinguishable representations or learning class-irrelevant spurious features, etc }

% I think in this paragraph, we want to clarify that while class collapse has technically been studied before, that analysis is useless because it cannot explain class collapse on population. to be able to explain class collapse / feature suppresion on population, we must figure out feature learning. tldr: our observation that feature learning must be dealt with is key differentiating factor from prior work. 
Addressing the above shortcomings requires theoretical understanding of how contrastive learning learns semantically meaningful features from the data \sj{why?}.  Nevertheless, existing studies are mostly limited to analyzing the error of downstream tasks under variety of assumptions 
\cite{arora2019theoretical, cl_theory_saunshi_2019, tosh2021contrastive,haochen2021provable,huang2021towards},
\yx{i think we should either not mention these works here (but leave them to the related work), or make it clear that they are not about CC or FS. }
or studying the geometrical properties of the representations obtained by minimizing the contrastive loss 
\cite{wang2020understanding,cc_dissecting_scl_2021,huang2021towards}. \yx{`The only work we notice that has theoretical studied class collapse is \citet{cc_dissecting_scl_2021} and there is no theoretical formulation of feature suppression.'}
Such studies do not provide any insights on the feature learning mechanism of contrastive learning \sj{and thus cannot explain the aforementioned failure modes?}. Understanding how CL learns features of the training data requires developing new sets of analysis tools that allows incorporating: properties of the model, effect of data augmentation, and most importantly the properties of the optimization algorithm.

% \yx{rephrase the paragraph and replace test set class collapse with `poor representation on test set?'} To address these challenges, it is essential to theoretically understand them. However, feature suppression has no existing theoretical formulation, and prior theoretical work on class collapse \cite{cc_dissecting_scl_2021} fails to distinguish between class collapse on training set and test set. Thus, no existing theory can explain why contrastive learning leads to models that suffer from class collapse or feature suppression on previously unseen data. 

% \PYB{By 'unseen data' do we mean unseen data that were drawn from the same data distribution as seen (training) data? \sj{yes, same distribution, just not seen. same distribution test data is what we want to talk about here}}

% Recent works on class collapse \cite{cc_dissecting_scl_2021} posit that minimizing the supervised contrastive loss leads to representations for each class collapsing to the vertices of a regular simplex. However, these analyses make no reference to the data distribution, model or training algorithm. \ba{what's the issue if they don't make a reference?} Similarly for feature suppression, while there is no prior theoretical characterization, \cite{chen2021intriguing} explains it as a property of the unsupervised contrastive loss. However, this raises the question, \textit{can the value of the loss function and the geometry of embeddings on the training set be used, in isolation, to explain class collapse and feature suppression?} We show that  any such explanation is vacuous since with over-parameterized models (akin to the architectures used in modern deep learning), the model minimizing the loss is not unique.  \looseness=-1

% The challenge in characterizing these phenomena on the test set is determining whether or not a given feature is learnt by the model. In particular, for class collapse, we must ascertain whether or not sub-class features are learnt; while for feature suppression, whether or not semantically meaningful features are learnt. 
%However, for class collapse, there is a unique embedding that minimizes the loss on training set, however, there exist many models that implement this embedding. For feature suppression, even the optimal embedding is not unique. 
% Any framework agnostic to the input and/or model obviously cannot make claims about which features are learnt by the model. Hence, any such analysis \cite{cc_dissecting_scl_2021} cannot truly characterize class collapse or feature suppression on unseen data. 

%Critically, we show that is impossible to explain these phenomena without accounting for the role of inductive bias by constructing global minimizers of the loss functions that select for different features. 

%We confirm this, empirically, by training models that do not suffer from class collapse and \textit{feature suppression} respectively, while achieving identical training loss as their counterparts that are plagued by these problems. Surprisingly, we find, both theoretically and empirically, that even when class collapse does occur subclass features are learnt early in training. Finally, we also show that our theoretical analysis can be used to understand why in practice training with a joint supervised and unsupervised contrastive loss \cite{islam2021broad,cc_chen2022perfectlybalanced} can be helpful. 

We address the above challenges by developing the first rigorous analysis framework that enables understanding the feature learning mechanism of CL, by taking into account properties of the model, data augmentation, and optimization algorithm.\yx{drop `optimization algorithm' and insert `... reveal the importance of considering inductive bias of training algorithms' at (*)?}\ba{inductice bias is only for sgd, I'm not sure it's defined in general for any optimization algorithm. Also we say "properties"} \yx{i think in general it usually refers to the (conjectured) regularization the algorithm provides}We leverage our framework to characterize the conditions that result in class collapse or feature suppression while learning representations of the training examples \yx{(*)}. 
We summarize our contributions below.

% and present a rigorous characterization of feature learning in contrastive learning. This, in turn, enables our analysis to determine when class collapse and feature suppression will occur on unseen data. \yx{the first sentence is something stronger than the second sentence, so how do we bring that across, maybe we can remove second sentnce?}

%\ba{this numbered list is more distracting than helpful to me. I'd summarize all the class collapse results in 1 paragraph and those of feature suppression in another paragraph (and you can number things within the paragraph).}

% \sj{somewhere we should say that when we talk about class collapse, we are talking about test set class collapse / class collapse on population}

% \PYB{We may need to briefly explain what 'inductive bias' is}

\textbf{Class Collapse in Supervised CL.} We show that, perhaps surprisingly and in contrast to the current understanding \cite{cc_dissecting_scl_2021}, global minimizers of the supervised contrastive loss does not necessarily collapse the representations of the subclasses %on unseen data 
at \textit{test} time. In fact, only \yx{we didn't show `only' min norm can result in cc. how about `however, the min norm minimizer can result in xxx'} the \textit{minimum norm} minimizer results in collapsing the subclass representations of the test data. 
Interestingly, we show that minimizing the contrastive loss using (stochastic) gradient descent (SGD) first learns the subclass features. However, as training proceeds, SGD\yx{(S)GD?} forgets the learned subclass features and collapses the subclass representations.
Our results are in line with recent studies revealing the bias of SGD towards finding simpler solutions \cite{lyu2021gradient}, and indicate it as the main deriving factor in collapsing the subclass representations.

% prove that when trained with gradient descent, subclass features are actually learnt early in training. Empirically, we observe that contrastive learning trained with (stochastic) gradient descent, initially learns subclass features, but then proceeds to unlearn them, resulting in class collapse. %Further, we show that while not all global minimizers of the loss have class collapse, the minimum norm minimizer does suffer from class collapse. Thus, we conjecture that (stochastic) gradient descent has an inductive bias towards simplicity (e.g. minimum norm solution) leading to class collapse.  

\textbf{Feature Suppression in Unsupervised CL.} %Using our feature learning framework, 
We provide the first theoretical characterization of feature suppression in unsupervised contrastive learning. In particular, we show that the minimum norm solution of the contrastive loss results in feature suppression, when the embeddings dimensionality is small \textit{or} when data augmentations preserve class-irrelevant features better than the semantically-relevant class features. 
Again, our results identifies the simplicity bias of SGD as a key factor in suppressing features of the input data. 
In addition, our analysis demonstrate the importance of taking into account properties of the model, such as dimensionality of the embeddings, as well as properties of data augmentation.
% feature suppression can be caused by an inductive bias towards simplicity (e.g. minimum norm solution) and \yx{rephrase}: (1) limited embedding space or (2) imperfect data augmentations. 

\textbf{Leveraging Supervised and Unsupervised CL to Obtain Superior Representations.} 
Finally, we prove that contrastive representation learning using a linear combination of supervised and unsupervised contrastive loss does not suffer from class collapse or feature suppression, even when minimized with (stochastic) gradient descent. Our results \sj{provide the first theoretical understanding of the benefits of such a joint loss} for learning higher-quality representations via the commonly-used stochastic gradient methods. \looseness=-1

% We further demonstrate the utility of our feature learning framework to rigorously justify why the joint supervised and unsupervised contrastive loss can avoid both class collapse and feature suppression, 
% % \yx{can we be less specific. for example why the joint supervised and unsupervised contrastive loss can outperform individual loss}, 
% despite the usual inductive bias towards simplicity. 
